Inf-DiT: Upsampling Any-Resolution Image with Memory-Efficient Diffusion Transformer

Diffusion models have shown remarkable performance in image generation in recent years. However, due to a quadratic increase in memory during generating ultra-high-resolution images (e.g. 4096*4096), the resolution of generated images is often limited to 1024*1024. In this work. we propose a unidirectional block attention mechanism that can adaptively adjust the memory overhead during the inference process and handle global dependencies. Building on this module, we adopt the DiT structure for upsampling and develop an infinite super-resolution model capable of upsampling images of various shapes and resolutions. Comprehensive experiments show that our model achieves SOTA performance in generating ultra-high-resolution images in both machine and human evaluation. Compared to commonly used UNet structures, our model can save more than 5x memory when generating 4096*4096 images. The project URL is https://github.com/THUDM/Inf-DiT.

==> sections/4_experiment_review.tex <==
 % \vspace{-2mm}
\section{Experiments}
% This section outlines our training process and subsequent comparative experiments, which include machine and human evaluations. We comprehensively compare Inf-DiT, our super-resolution enhanced ultra-high-resolution generation model, against existing models in both domains.

In this section, we first introduce the detailed training process of Inf-DiT, then comprehensively evaluate Inf-DiT by both machine and human evaluation. The results show that Inf-DiT surpasses all baselines, excelling in both ultra-high-resolution image generation and upsampling tasks. Finally, we conduct ablation studies to validate the effectiveness of our design.

% We conducted quantitative comparisons of the Inf-DiT against state-of-the-art methodologies over two tasks: 1. ultra-high-resolution image generation condition on text, and 2. image super-resolution. In the domain of ultra-high-resolution generation, our Inf-DiT was benchmarked against Direct Inference, MultiDiffusion, SDXL$+$BSRGAN, SDXL$+$Real-ESRGAN, ScaleCrafter, and Demofusion. These comparisons were anchored on the HPDv2 (Human Preference Dataset v2)\cite{wu2023human} benchmark dataset, with the aim of mitigating bias to secure more reliable and equitable evaluation outcomes, thereby ensuring alignment with human ethics and decision-making processes. For the super-resolution task, the Inf-DiT's performance was evaluated in comparison with LDM, StableSR, BSRGAN, and Real-ESRGAN, specifically leveraging the DIV2k\_valid\cite{agustsson2017ntire} dataset for this assessment. Furthermore, considering that the assessment of high-resolution images cannot be entirely quantified through machine evaluation, we further conduct a user study on HPDv2 dataset.

%FID	3200-2048	3200-2048-patch	3200-4096	3200-4096-patch	mean
% bsr	68.1 	85.5 	66.0 	85.0 	76.2 
% our_clip0	66.3 	74.7 	67.0 	76.2 	71.1 
% scalecrafter	79.9 	95.5 	115.1 	153.3 	111.0 
% demofusion	67.5 	72.0 	70.8 	82.6 	73.2 
% esr	68.0 	77.0 	65.6 	78.1 	72.2 
% direct	92.2 	92.3 			92.3 
% multidiffusion	99.7 	109.3 			104.5 
% our1024t2048 09	66.1 	70.7 			
% demo09	68.0 	71.0 			
% esr 10 2scale	66.7 	75.0 			
% bsr 10 2scale	66.3 	81.7 			
% ema 10	66.4 	76.3 			
% our1024t2048 10	66.0 	71.9 			
% SDXL+Real-ESRGAN & $66.7$ & $75.0$ & $\textbf{65.6}$ & $78.1$ & $71.4$ \\
					
% DIV2k_valid	FID	patch-fid	PNSR	SSIM
% variable resolution				
% our_clip0	20.2 	76.5 	26.3 	0.74 
% bsr	35.0 	143.2 	25.9 	0.73 
% esr	35.5 	127.6 	25.2 	0.72 
% Fix resolution(512*512)				
% our_clip0	38.6 	83.3 	24.6 	0.67 
% stablesr	74.8 	112.6 	22.0 	0.60 
% Fix resolution(256*256)				
% our_clip0	86.8 	-	24.6 	0.67 
% ldm	152.6 	-	23.9 	0.66 


% \begin{table}[h!]
% \centering
% \resizebox{\textwidth}{!}{% Resize table to fit within the text width
% \begin{tabular}{@{}llllllllllll@{}}
% \toprule
% & \multicolumn{2}{c}{2048 x 2048} & \phantom{abc} & \multicolumn{2}{c}{2048 x 4096} & \phantom{abc} & \multicolumn{2}{c}{4096 x 4096} \\
% \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
% Method & FID$\downarrow$ & IS$\uparrow$ && FID$_{\text{crop}}\downarrow$ & IS$_{\text{crop}}\uparrow$ & CLIP$\uparrow$  & FID$\downarrow$  \\ 
% \midrule
% SDXL Direct Inference [24] & 79.66 & 13.47 && 73.91 & 17.38 & 28.12 & 97.08 & 14.12 & 27.29 \\
% MultiDiffusion [2] & 75.93 & 14.56 && 70.93 & 17.85 & 28.97 & 89.38 & 14.17 & 28.66  \\
% SDXL + BSRGAN [39] & 66.41 & 16.22 && 67.42 & 21.11 & 29.61 & 68.70 & 16.29 & 29.01  \\
% SCALECRAFTER [7] & 69.91 & 15.72 && 68.36 & 19.44 & 29.51  & 80.16 & 15.20 & 28.87  \\
% Ours & 65.73 & 16.41 && 64.81 & 21.40 & 29.68 & 73.15 & 16.11 & 29.05  \\
% \bottomrule
% \end{tabular}
% }
% \caption{Your caption here.}
% \label{tab:my_label}
% \end{table}
% \noindent % 确保从页面边缘开始
% \begin{minipage}{.6\linewidth}
% \centering

% \end{minipage}%
% \hspace{2mm} % 添加2mm的水平空间
% \begin{minipage}{.4\linewidth}
% \centering
 \vspace{-5mm}
\begin{table*}[htbp]
    \renewcommand{\arraystretch}{1}
    \caption{Quantitative comparison results with state-of-the-art methods of ultra-high-resolution generation on HPDV2 dataset. The best results are marked in \textbf{bold}, and the second best results are marked by \underline{underline}.}
    \centering
    \begin{adjustbox}{width=\linewidth,center}
    \setlength{\tabcolsep}{11.5pt}
    \begin{tabular}{c|cc|cc|c}
    \toprule[1pt]
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{$2048 \times 2048$} & \multicolumn{2}{c|}{$4096 \times 4096$} & \multirow{2}{*}{\textbf{Mean} $\downarrow$} \\
    \cline{2-5} & \rule{0pt}{2.6ex}FID $\downarrow$  & FID$_{\text{crop}}$ $\downarrow$  & FID $\downarrow$  & FID$_{\text{crop}}$ $\downarrow$  & \\
    \midrule[1pt]
        Direct Inference & $92.2$ & $92.3$ & OOM & OOM & $92.3$ \\
        MultiDiffusion & $99.7$ & $109.3$ & OOM & OOM & $104.5$ \\
        SDXL+BSRGAN & $\underline{66.3}$ & $81.7$ & $\textbf{66.0}$ & $85.0$ & $74.8$ \\
        ScaleCrafter & $79.9$ & $95.5$ & $115.1$ & $153.3$ & $111.0$ \\
        DemoFusion & $67.5$ & $\underline{72.0}$ & $70.8$ & $\underline{82.6}$ & $\underline{73.2}$ \\
        SDXL+Inf-DiT(Ours) & $\textbf{66.0}$ & $\textbf{71.9}$ & $\underline{67.0}$ & $\textbf{76.2}$ & $\textbf{70.3}$ \\
    \midrule[1pt]
    \end{tabular}
    \end{adjustbox}
    \vspace{0.1mm}
    \label{tbl:comparison}
     \vspace{-1mm}
    \end{table*}
\vspace{-10mm}
% \end{minipage}%
% \hspace{2mm} % 添加2mm的水平空间
% \begin{minipage}{.4\linewidth}
% \centering
\begin{table*}[htbp]
    \renewcommand{\arraystretch}{1}
    \caption{Quantitative comparison results with state-of-the-art methods of super resolution on DIV2K dataset. The best results are marked in \textbf{bold}.}
    \centering
    \begin{adjustbox}{width=\linewidth,center}
    \setlength{\tabcolsep}{8.5pt}
    \begin{tabular}{c|c|cccc}
    \toprule[1pt]
      \textbf{Setting} & \textbf{Method} & FID $\downarrow$ & FID$_{\text{crop}}$ $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ \\
    \midrule[1pt]
     \multirow{3}{*}{Variable resolution} & BSRGAN & 35.0 & 143.2 & 25.9 & 0.73 \\
     & Real-ESRGAN & 35.5 & 127.6 & 25.2 & 0.72 \\
     & Inf-DiT(Ours) & \textbf{20.2} & \textbf{76.5} & \textbf{26.3} & \textbf{0.74} \\
    \midrule[0.5pt]
     \multirow{2}{*}{Fix resolution (512x512)} & StableSR & 74.8 & 112.6 & 22.0 & 0.60  \\
     & Inf-DiT(Ours) & \textbf{38.6} & \textbf{83.3} & \textbf{24.6} & \textbf{0.67}\\
    \midrule[0.5pt]
     \multirow{2}{*}{Fix resolution (256x256)} & LDM & 152.6 & - & 23.9 & 0.66 \\
     & Inf-DiT(Ours) & \textbf{86.8} & - & \textbf{24.6} & \textbf{0.67} \\
    \bottomrule[1pt]
    \end{tabular}
    \end{adjustbox}
    \vspace{0.1mm}
    \label{tbl:resolution_comparison}
     \vspace{-5mm}
\end{table*}
% \end{minipage}%

% \begin{figure}[htbp]
%   \centering
%   \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{images/compare/StableSR.jpg}
%     \caption{Patch method}
%     \label{fig:image1}
%   \end{subfigure}
%     \hfill % optional; add some horizontal spacing
%   \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{images/compare/esrgan.jpg}
%     \caption{esrgan}
%     \label{fig:image2}
%   \end{subfigure}
%   \hfill % optional; add some horizontal spacing
%   \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{images/compare/demofusion.jpg}
%     \caption{demofusion}
%     \label{fig:image2}
%   \end{subfigure}
%   \hfill % optional; add some horizontal spacing
%   \begin{subfigure}[b]{0.24\textwidth}
%     \includegraphics[width=\textwidth]{images/compare/ours.jpg}
%     \caption{ours}
%     \label{fig:image2}
%   \end{subfigure}
%   \caption{comparison}
%   \label{fig:images}
% \end{figure}

%Watchout!!!!!!Remember to check if we say Real-ESRGAN. (No ESRGAN)!!!

% \FloatBarrier




\subsection{Training Details}

\subsubsection{Datasets}

Our dataset comprises a subset of LAION-5B\cite{schuhmann2022laionb} with a resolution higher than $1024\times1024$ and aesthetic score higher than 5, and 100 thousand high-resolution wallpapers from the Internet.
Following the previous works\cite{saharia2022photorealistic, ramesh2022hierarchical, wang2021real}, we use fixed-size image crops of $512 \times 512$ resolution during training. Since upsampling can be conducted with local information only, it can be directly employed at higher resolution during inference, which is not easy for most generation models. % 解释为什么训练推理可以不一样分辨率？
 \vspace{-5mm}
\subsubsection{Data Processing}
Since the images generated by diffusion models often contain residual noise and various detail inaccuracies, it becomes crucial to enhance the robustness of the upsampling model to address these issues. We adopt the approach similar to Real-ESRGAN\cite{wang2021real} to perform a variety of degradation on low-resolution input images within the training data. 

When processing training images with a resolution higher than 512, there are two alternative methods: directly performing a random crop, or resizing the shorter side to 512 before performing a random crop. While the direct cropping method preserves high-frequency features in high-resolution images, the resize-then-crop method avoids frequently cropping out areas with a single color background, which is detrimental to the model's convergence. Therefore, in practice, we randomly select from these two processing methods to crop training images. 

% When processing training set images with a resolution greater than 512, there are two alternative methods: resizing the shorter side to 512 before performing a random crop or directly performing a random crop. 
% It can be observed that in internet image datasets like LAION-5B, the distribution of 512-sized patches cropped from high-resolution images significantly differs from the distribution of images whose edges are exactly 512 pixels, as demonstrated in Figure xx. We define these textures and patterns, present only in slices from high-resolution images, as high-frequency details. Most of these high-frequency details are lost when downsampling the entire image.

% To ensure that models trained at 512 resolution can infer at higher resolutions, learning those high-frequency details is essential. However, performing a random crop on large images can easily result in cropping out areas with a single color background, which is detrimental to the model's convergence speed. Therefore, in practice, one of the two processing methods is randomly selected to generate training data of size 512.
 \vspace{-5mm} %``''引号
\subsubsection{Training settings}
During training, We set $block \ size=128$ and $patch\  size=4$, which means every training image is divided into $4\times4$ blocks and every block has $32\times 32$ patches. 
We employ the framework of EDM\cite{karras2022elucidating} for training, and set the upsampling factor to $4 \times$. Because the upsampling task is more concerned with the high-frequency details of images, we adjusted the mean and std of training noise distribution to $-1.0$ and $1.4$. To address overflow problem during training, we employed BF16 format due to its broader numerical range. Our CLIP model is a ViT-L/16 pre-trained on Datacomp dataset\cite{ilharco_gabriel_2021_5143773}. Since the CLIP can only process images with $224 \times 224$ resolution, we first resize LR images to $224 \times 224$ and then input them to CLIP.
% Other hyperparamers are shown in\Cref{Hyperparam}.
Other hyperparameters are listed in the \cref{sec:appendix:imp}. 

\begin{figure}
\centering
% 第一排
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/direct_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/comb_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/scale_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/bsr_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/demo_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/ours_with_box.jpg}
\end{subfigure}
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/direct_zoomed.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/comb_zoomed.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/scale_zoomed.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/bsr_zoomed.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/demo_zoomed.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_woman2/ours_zoomed.jpg}
\end{subfigure}
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/direct_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/comb_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/scale_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/bsr_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/demo_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/ours_with_box.jpg}
\end{subfigure}
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/direct_zoomed.jpg}
  {\scriptsize\textbf{Direct}}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/comb_zoomed.jpg}
  {\scriptsize\textbf{Patch}}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/scale_zoomed.jpg}
  {\scriptsize\textbf{Scalecrafter}}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/bsr_zoomed.jpg}
  {\scriptsize\textbf{BSRGAN}}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/demo_zoomed.jpg}
  {\scriptsize\textbf{Demofusion}}
\end{subfigure}%
\begin{subfigure}{.14\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/compare_cat/ours_zoomed.jpg}
  % \caption{{\fontsize{2pt}{6pt}\selectfont Inf-DiT(Ours)}}
  {\scriptsize\textbf{Inf-DiT}}
\end{subfigure}%
\captionsetup{skip=2pt}
\caption{Qualitative comparison of different methods in detail at $2048\times2048$ resolution}
\label{fig:images}
\vspace{-4mm}
\end{figure}
 % \vspace{-100mm}
 % \vspace{-5mm}
\begin{figure}[!h]
\centering
% 第一排
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/lionpaper/comb_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/lionpaper/scale_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/lionpaper/bsr_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/lionpaper/demo_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/lionpaper/ours_with_box.jpg}
\end{subfigure}
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/lionpaper/comb_zoomed.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/lionpaper/scale_zoomed.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/lionpaper/bsr_zoomed.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/lionpaper/demo_zoomed.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/lionpaper/ours_zoomed.jpg}
\end{subfigure}
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/man2paper/patch_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/man2paper/scale_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/man2paper/bsr_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/man2paper/demo_with_box.jpg}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/man2paper/ours_with_box.jpg}
\end{subfigure}
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/man2paper/patch_zoomed.jpg}
  {\scriptsize\textbf{Patch}}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/man2paper/scale_zoomed.jpg}
  {\scriptsize\textbf{Scalecrafter}}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/man2paper/bsr_zoomed.jpg}
  {\scriptsize\textbf{BSRGAN}}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/man2paper/demo_zoomed.jpg}
  {\scriptsize\textbf{Demofusion}}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[width=\linewidth]{images/man2paper/ours_zoomed.jpg}
  {\scriptsize\textbf{Inf-DiT}}
\end{subfigure}%
\captionsetup{skip=2pt}
\caption{{Qualitative comparison of different methods in detail at $4096\times4096$ resolution}}
\label{fig:images}
 \vspace{-7mm}
\end{figure}

\subsection{Machine Evaluation}
In this part, we conduct quantitative comparisons of Inf-DiT against state-of-the-art methodologies on ultra-high-resolution image generation tasks. The baselines encompass two main categories of high-resolution generation: 1. Direct high-resolution image generation, including Direct Inference of SDXL\cite{podell2023sdxl}, MultiDiffusion~\cite{bar2023multidiffusion}, ScaleCrafter~\cite{he2023scalecrafter}, and 2. High-resolution image generation based on super-resolution techniques, including BSRGAN~\cite{zhang2021designing}, %Real-ESRGAN~\cite{wang2021real}, 
DemoFusion~\cite{du2023demofusion}. We employ the FID (Fr\'echet Inception Distance)~\cite{heusel2017gans} to evaluate the quality of ultra-high-resolution generation, which is widely used to evaluate the perceptual quality of images in image generation tasks \cite{rombach2022high,peebles2023scalable,saharia2022photorealistic}. To further validate the super-resolution ability of our model, we additionally benchmark it against renowned super-resolution models over classic super-resolution tasks. 

 % \vspace{-5mm}
% 我们进行对比实验，比较对象包含了超分辨率生成两个主要的类别：1.2. 首先进行了FID测评，FID为什么好？其次补充了超分测评实验。
\subsubsection{Ultra-High-Resolution Generation} \label{subsubsec:exp-high-generation}

We use the test set of HPDv2\cite{wu2023human} for evaluation. It contains 3200 prompts and is divided into four categories: ``Animation'', ``Concept-art'', ``Painting'', and ``Photo''. This allows for a comprehensive evaluation of the model's generative capabilities across various domains and styles. We test on two resolutions: $2048^2 $ and $4096^2$. For super-resolution-based models, we first use SDXL to generate a $1024^2$ resolution image and upsample it without text. We use $2 \times $ and $4 \times$ versions of BSRGAN for $2048^2$ and $4096^2$ generation, respectively. Although Inf-DiT was trained in a setting with $4 \times$ upsample, we find that it can generalize well at lower upsampling multiples. % 啥意思
Therefore, for $2048^2$ generation, we directly resize the LR image from $1024^2$ to $2048^2$ and concatenate it with the noise input. We random samples 3200 images of $2048^2$ and $4096^2$ from LAION-5B as the distribution of real images.


As for the metrics, FID is designed to assess how closely generated images mimic real image distributions, and has become one of the default metrics in evaluating image generation. However, the original implementation of FID needs to downsample the input image to the resolution of $299\times299$ before the feature extraction, which ignores high-resolution details and can be inaccurate in assessing ultra-high-resolution image generation. Therefore, inspired by \cite{chai2022any,du2023demofusion}, we adopted the idea of $\text{FID}_{\text{crop}}$ and randomly crops $299\times299$ patches from high-resolution images for FID evaluation. Still, we retain the FID metric as it serves as an indicator of overall consistency, which the $\text{FID}_{\text{crop}}$ might overlook.

% \begin{table*}[htbp]
%     \renewcommand{\arraystretch}{1}
%     \caption{\textbf{Quantitative comparison results}. The best results are marked in \textbf{bold}.}
%     \centering
%     \begin{adjustbox}{width=\linewidth,center}
%     \setlength{\tabcolsep}{11.5pt}
%     \begin{tabular}{c|cc|cc|c}
%     \toprule[1pt]
%     \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{$2048 \times 2048$} & \multicolumn{2}{c|}{$4096 \times 4096$} & \multirow{2}{*}{\textbf{Mean}} \\
%     \cline{2-5} & \rule{0pt}{2.6ex}FID  & FID$_{\text{crop}}$  & FID  & FID$_{\text{crop}}$  & \\
%     \midrule[1pt]
%         Direct Inference & $92.2$ & $92.3$ & OOM & OOM & $92.3$ \\
%         MultiDiffusion & $99.7$ & $109.3$ & OOM & OOM & $104.5$ \\
%         SDXL+BSRGAN & $66.3$ & $81.7$ & $66.0$ & $85.0$ & $74.8$ \\
%         SDXL+Real-ESRGAN & $66.7$ & $75.0$ & $\textbf{65.6}$ & $78.1$ & $71.4$ \\
%         ScaleCrafter & $79.9$ & $95.5$ & $115.1$ & $153.3$ & $111.0$ \\
%         DemoFusion & $67.5$ & $72.0$ & $70.8$ & $82.6$ & $73.2$ \\
%         Inf-DiT(Ours) & $\textbf{66.0}$ & $\textbf{71.9}$ & $67.0$ & $\textbf{76.2}$ & $\textbf{70.3}$ \\
%     \midrule[1pt]
%     \end{tabular}
%     \end{adjustbox}
%     \vspace{0.1mm}
%     \label{tbl:comparison}
%     \end{table*}
% \vspace{-10mm}



% As for the evaluation dataset, we use the test set of HPDv2\cite{wu2023human}, which contains 3200 prompts and is divided into four categories: "Animation", "Concept-art", "Painting", and "Photo". This allows for a comprehensive evaluation of the model's generative capabilities across various domains and styles. For super-resolution-based models, we first use SDXL to generate a $1024\times1024$ resolution image and upsampling it without text. We use $2 \times $ and $4 \times$ versions of BSRGAN and RealESRGAN for 2048 and 4096 generation, respectively. Although Inf-DiT was trained in a setting with $4 \times$ upsample, we find that it can generalize well at lower multiples. Therefore, for 2048 generation, we directly resize the LR image from 1024 to 2048 and concatenate it with the noise input.    

 The results in \cref{tbl:comparison} demonstrate that our model achieves state-of-the-art (SOTA) in three out of four metrics and surpasses all competitors in the mean score. This showcases our model's exceptional ability to generate high-resolution details and harmonious global information. The sole exception is the FID at $4096^2$, where it marginally trail behind BSRGAN by 1.0, but as discussed above, $\text{FID}_{\text{crop}}$ is a more representative metric for high-resolution features and Inf-DiT surpasses BSRGAN on $\text{FID}_{\text{crop}}$ on both $2048^2$ and $4096^2$ resolution. Our model is capable of being applied to all generative models, not just SDXL. Examples of upsampled images from other models are listed in the \cref{sec:appendix:morecase}. 
 
  % \vspace{-7.4mm}
\subsubsection{Super-Resolution}
In addition to its ability to generate high-resolution images, Inf-DiT can also be used as a classic super-resolution model. We conduct the evaluation on DIV2k valid dataset\cite{agustsson2017ntire} which contains multiple real-world high-resolution images in different scenarios. Following \cite{rombach2022high, saharia2022image}, we fix image degradation to bicubic interpolation with $4 \times$ downsampling. Before comparing with fix-resolution models LDM\cite{rombach2022high} and StableSR\cite{wang2023exploiting}, we center-crop specific-sized patches from the high-resolution image as ground truth.
% The work is twofold: 1. For resolutions without predefined targets, we apply 4x downsampling to the original dataset images, then conduct 4x super-resolution, comparing our results with BSRGAN and Real-ESRGAN. 2. For fixed-resolution tasks, we extract specific-sized patches, apply 4x super-resolution, and benchmark against StableSR at $512\times512$ resolution and LDM at $256\times256$ resolution. 
Throughout this process, we utilize both perceptual (FID, $\text{FID}_{\text{crop}}$) and fidelity (PSNR, SSIM) metrics to ensure a detailed and comprehensive assessment.

% \begin{table*}[htbp]
%     \renewcommand{\arraystretch}{1}
%     \caption{\textbf{Quantitative comparison results}. The best results are marked in \textbf{bold}.}
%     \centering
%     \begin{adjustbox}{width=\linewidth,center}
%     \setlength{\tabcolsep}{8.5pt}
%     \begin{tabular}{l|l|cccc}
%     \toprule[1pt]
%       Setting & Method & FID $\downarrow$ & FID$_{\text{crop}}$ $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ \\
%     \midrule[1pt]
%      \multirow{3}{*}{Variable resolution} & BSRGAN & 35.0 & 143.2 & 25.9 & 0.73 \\
%      & Real-ESRGAN & 35.5 & 127.6 & 25.2 & 0.72 \\
%      & Inf-DiT(Ours) & \textbf{20.2} & \textbf{76.5} & \textbf{26.3} & \textbf{0.74} \\
%     \midrule[0.5pt]
%      \multirow{2}{*}{Fix resolution (512x512)} & StableSR & 74.8 & 112.6 & 22.0 & 0.60  \\
%      & Inf-DiT(Ours) & \textbf{38.6} & \textbf{83.3} & \textbf{24.6} & \textbf{0.67}\\
%     \midrule[0.5pt]
%      \multirow{2}{*}{Fix resolution (256x256)} & LDM & 152.6 & - & 23.9 & 0.66 \\
%      & Inf-DiT(Ours) & \textbf{86.8} & - & \textbf{24.6} & \textbf{0.67} \\
%     \bottomrule[1pt]
%     \end{tabular}
%     \end{adjustbox}
%     \vspace{0.1mm}
%     \label{tbl:resolution_comparison}
%      \vspace{-5mm}
% \end{table*}

As demonstrated in \cref{tbl:resolution_comparison}, our model achieves state-of-the-art (SOTA) across all metrics. This signifies that, as a super-resolution model, ours not only excels in performing super-resolution at arbitrary scales but also in optimally preserving global and detailed information while restoring results that closely resemble the original images.
% \vspace{-5mm}
\subsection{Human Evaluation}
To further evaluate Inf-DiT and more accurately reflect its generative quality from a human perspective, we conduct a human evaluation. The comparison settings are the same as in \cref{subsubsec:exp-high-generation}, except that we excluded MultiDiffusion and Direct Inference to their non-competitive results. For each of the four categories, we randomly choose ten comparison sets, each encompassing outputs from four models, culminating in a total of 40 sets that form the human evaluation dataset. To ensure fairness, we randomize the sequence of model outputs in each comparison set. Human evaluators are asked to evaluate models based on three criteria: detail authenticity, global coherence, and consistency with the original low-resolution input. Each evaluator receives 20 sets of images on average. Within each set, evaluators are required to rank the images generated by four models from highest to lowest based on three criteria. 

% The user study adopted the same comparison format as the quantitative comparison for ultra-high-resolution generation. The participating models for comparison remained the same, with the exception of MultiDiffusion and Direct Inference, which were excluded due to their non-competitive results. In the collection of $2048\times2048$ images generated earlier, ten sets per category were chosen at random, culminating in a total of 40 sets that form the basis of the human evaluation dataset. Each set encompasses outputs from five models, the $1024\times1024$ results directly generated by SDXL and the original prompt. To ensure impartiality, the sequence of model outputs within each set is rigorously randomized.

We ultimately collected 3,600 comparisons. As depicted in \cref{fig:human_evalution_rank}, our model outperforms the other 3 methods in all the 3 criteria. It is particularly noteworthy that each of the other three models ranks relatively lower on at least one of the three evaluation criteria, while Inf-DiT achieves the highest score on all three criteria: detail authenticity, global coherence, and consistency with low-resolution input. This indicates that our model is the only one capable of excelling in both high-resolution generation and super-resolution tasks simultaneously.


% Note that we have not included aesthetic and artistic qualities of the images here as these criteria largely depend on the lower-resolution images rather than being the focus of ultra-high-resolution generation. 
% Conversely, the generation of details and overall control precisely represent the best quantitative measures of the genuine value that ultra-high-resolution generation can alter. 
% Furthermore, for evaluating the infinite-scale super-resolution approach, we have added original input consistency as a measure.


 \vspace{-16pt} % 向上移动接下来的文本或其他内容
\begin{figure}[h]
   \centering
   \includegraphics[width=\linewidth]{images/human_evaluation_rank.png}
   \captionsetup{skip=2pt}
   \caption{Human evaluation results. After participants rank the images from different models, We assign scores from 4 to 1 to models in order and finally calculate the average of all the results. Inf-DiT gets the highest scores in all three categories.}
   \label{fig:human_evalution_rank}
     \vspace{-9mm}
\end{figure}
 % \vspace{-27pt} % 向上移动接下来的文本或其他内容


\subsection{Iterative Upsampling}
\vspace{-2mm}


\begin{wraptable}[8]{r}{0.5\linewidth}
    \vspace{-14mm}
    \centering
    \caption{Ablation study on $2048 \times 2048$ resolution.}
    \begin{tabular}{ccc}
    \toprule
    Method & FID & $\text{FID}_\text{crop}$ \\
    \midrule
    Ours & \textbf{66.0} & \textbf{71.9} \\
    w/o Nearby LR Attention & 66.7 & 73.6 \\
    w/o Semantic Input & 66.2 & 72.8 \\
    Inner Block Attention & 66.3 & 83.7 \\
    \bottomrule
    \vspace{-15mm}
    \end{tabular}
    \label{tab:ablation_study}
\end{wraptable}

\begin{figure}[t]
   \centering
   \includegraphics[width=\linewidth]{images/interative_upsampling.jpg}
   \caption{Generated samples of iterative upsampling. \textbf{Top}: Inf-DiT can upsample an image generated by itself several times, and generate details of different frequencies at corresponding resolution. \textbf{Bottom}: After failing to generate a pupul at the $128^2$ resolution, it is difficult for subsequent upsampling stages to correct this error. }
   \label{fig:interative_upsampling}
    \vspace{-5mm}
\end{figure}
 % \vspace{-10pt}


Since our model can upsample images of arbitrary resolution, it's a natural idea to test if the model can iteratively upsample images generated by itself. In this study, we experiment on generating a $2048^2$ resolution image from a $32^2$ resolution image , $64 \times $ upscale, through three times of iterative upsampling. \Cref{fig:interative_upsampling} illustrates two cases of this process. In the first case, the model successfully produces a high-resolution image after three stages of upsampling. It generates details of different frequencies in different resolution upsampling: the contour of the face, the shape of the eyeball, and individual eyelashes. However, it is hard for the model to correct inaccuracies generated in earlier stages, leading to the accumulation of errors. An example of this issue is demonstrated in the second sample. We leave this problem for our future work.   


\subsection{Ablation Study}
We conduct ablation studies of our method on $2048^2$ resolution. We test the model performance on the HPDV2 dataset after separately removing the Global Input and Nearby LR attention. As a result, both the FID and $\text{FID}_{\text{crop}}$ of the model get worse to varying degrees. We also test Inner Block Attention setting, i.e. removing the attention between blocks,  and the $\text{FID}_{\text{crop}}$ experiences a significant decline. We list more case studies and analysis in the \cref{sec:appendix:abcases}. 
% \begin{wraptable}{r}{5cm} % 假设表格宽度为5cm
%   \caption{Your caption here}
%   %\label{tab:abstudy}
%   \begin{tabular}{@{}ccc@{}}
%     \hline
%     Method & FID & $\text{FID}_\text{crop}$ \\
%     \hline
%     ours & 66.0 & 71.9 \\
%     w/o nearby lr attention & 66.7 & 73.6 \\
%     w/o global input & 66.2 & 72.8 \\
%     inner block attention & 66.3 & 83.7 \\
%     \hline
%   \end{tabular}
% \end{wraptable}


% A visual result of removing three key technical components, including timestep-wise progres- sive re-dilation (progression), convolution dis- persion, and noise-damped classifier-free guid- ance (nd-cfg), can be seen in Fig. 7. It high- lights that the timewise progressive decrease in perception field via re-dilation improves visual
%  Table 4: Ablation study on SD 1.5.
% quality, especially in image details. Noise-damped classifier-free guidance ensures less noise in the final image, and dispersed convolution improves the fidelity of object structures. Tab. 4 shows quantitative results. Without these components, the FID performance dropped by 16.68, 27.96, and 33.93, respectively. Therefore, every technical component of our method brings considerable improvements.

